DP-FP: Differentially Private Forward Propagation for Large Models

When applied to large-scale learning problems, the conventional wisdom on privacy-preserving deep learning, known as Differential Private Stochastic Gradient Descent (DP-SGD), has met with limited success due to significant performance degradation and high memory overhead when compared to the non-privacy counterpart. We show how to mitigate the performance drop by replacing the DP-SGD with a novel DP Forward-Propagation (DP-FP) followed by an off-the-shelf non-DP optimizer. Our DP-FP employs novel (1) representation clipping followed by noise addition in the forward propagation stage, as well as (2) micro-batch construction via subsampling to achieve DP amplification and reduce noise power to $1/M$, where $M$ is the number of micro-batch in a step. When training a classification model, our DP-FP with all of the privacy-preserving operations on the representation is innately free of gradient bias, total noise proportionally to model size, and memory issues in DP-SGD. As a result, our DP-FP outperforms cutting-edge DP-SGD while retaining the same level of privacy, and it approaches non-private baselines and significantly outperforms state-of-the-art DP-SGD variants. When applied to RoBERTa-large on four downstream tasks, for example, DP-FP achieves an average accuracy of 91.34\% with privacy budgets less than 3, representing a 3.81\% performance improvement over the state-of-the-art DP-SGD and only a 0.9\% loss compared to the non-private baseline but with a significantly lower privacy leakage risk.

==> backup.tex <==
% \begin{figure}[h]
% \centering
% \begin{gnuplot}[terminal=pdf,terminaloptions={font ",12" linewidth 3 size 3.4in,2.5in}]
% 	set grid
% 	set ylabel 'Accuracy'
% 	set xlabel 'Batch size (b)'
% 	set logscale x
% 	set xrange [16:256]
% 	set xtics 2
% 	set size 0.9
% 	set yrange [90.0:94.0]
% 	set key bottom right
% 	plot "figure/batch_size_data.txt" i 0 u 1:2 w lp dashtype 5 t "lr = 1e-5", \
% 	     "figure/batch_size_data.txt" i 0 u 1:3 w lp dashtype 2 t "lr = 1e-6", \
% 	     "figure/batch_size_data.txt" i 0 u 1:4 w lp dashtype 1 t "lr = 5e-6"
% 	   %  "figure/batch_size_data.txt" i 0 u 1:5 w lp t "lr = 1e-7"
% \end{gnuplot}
% \abovecaptionskip=1pt
% \caption{Accuracy curves for different batch size (b) on SST-2 development set.}
% \label{fig:batch_curve}
% \end{figure}


% \begin{figure}[h]
% \centering
% \begin{gnuplot}[terminal=pdf,terminaloptions={font ",12" linewidth 3 size 3.4in,2.5in}]
% 	set grid
% 	set ylabel 'Accuracy'
% 	set xlabel 'Clip norm (c)'
% 	set xrange [0.1:1.0]
% 	set xtics 0.2
% 	set size 0.9
% 	set yrange [84.0:94.0]
% 	set key bottom right
% 	plot "figure/clip_data.txt" i 0 u 1:2 w lp dashtype 5 t "lr = 1e-5", \
% 	     "figure/clip_data.txt" i 0 u 1:3 w lp dashtype 2 t "lr = 1e-6", \
% 	     "figure/clip_data.txt" i 0 u 1:4 w lp dashtype 1 t "lr = 5e-6"
% 	   %  "figure/batch_size_data.txt" i 0 u 1:5 w lp t "lr = 1e-7"
% \end{gnuplot}
% \abovecaptionskip=1pt
% \caption{Accuracy curves for different clip norm (c) on SST-2 development set.}
% \label{fig:clip_curve}
% \end{figure}





% \begin{table*}[htp!]
%     \centering
%     %\scalebox{0.85}{
%     \begin{tabular}{c|cc|cc|cc|cc|cc}
%     \hline
%     Method & \multicolumn{2}{c|}{MNLI} & \multicolumn{2}{c|}{QQP} & \multicolumn{2}{c|}{QNLI} & \multicolumn{2}{c|}{SST-2} & \multicolumn{2}{c}{Avg.} \\
%     \hline
%     \cite{yu2021large} & - & 78.6 & - & 84.8 & - & 86.2 & - & 91.5 & - & 85.28\\
%     \cite{li2021large} & 82.29 & 83.22 & 85.41 & 86.15 & 84.62 & 84.81 & 86.12 & 85.89 & 84.61 & 85.02\\
%     \hline
%     Ours-Bert & 76.80 & 78.65 & 86.40 & 86.95 & 84.88 & 85.77 & 87.50 & 89.79 & 83.90 & 85.29\\
%     Ours-RoBerta & 79.36 & 81.65 & 85.49 & 86.87 & 84.09 & 86.00 & 82.91 & 87.84 & 82.96 & 85.59\\
%     \hline
%     N.P. Bert & \multicolumn{2}{c|}{84.52} & \multicolumn{2}{c|}{90.65} & \multicolumn{2}{c|}{90.61} & \multicolumn{2}{c|}{92.31} & \multicolumn{2}{c}{89.52}\\
%     \hline
%     N.P. RoBerta & \multicolumn{2}{c|}{86.19} & \multicolumn{2}{c|}{91.20} & \multicolumn{2}{c|}{91.64} & \multicolumn{2}{c|}{93.69} & \multicolumn{2}{c}{90.68}\\
%     \hline
%     \hline
%     $\epsilon =$ (MA) & 3 & 8 & 3 & 8 & 3 & 8 & 3 & 8 & 3 & 8\\
%     \hline
%     $\epsilon \approx$ (GDP+CLT) & 2.52 & 5.83 & 2.53 & 5.85 & 2 & 4.75 & 1.73 & 4.33 & <2.53 & <5.85\\
%     \hline
%     \end{tabular}
%     \caption{Performance comparison with DP-SGD in~\cite{li2021large}}
%     \label{table: DPSGD}
% \end{table*}


% \begin{table*}[htp!]
%     \centering
%     %\scalebox{0.85}{
%     \begin{tabular}{c|cc|cc|cc|cc|cc}
%     \hline
%     Method & \multicolumn{2}{c|}{MNLI} & \multicolumn{2}{c|}{QQP} & \multicolumn{2}{c|}{QNLI} & \multicolumn{2}{c|}{SST-2} & \multicolumn{2}{c}{Avg.} \\
%     \hline
%     \cite{yu2021large} & - & 78.6 & - & 84.8 & - & 86.2 & - & 91.5 & - & 85.28\\
%     \cite{li2021large} & 82.29 & 83.22 & 85.41 & 86.15 & 84.62 & 84.81 & 86.12 & 85.89 & 84.61 & 85.02\\
%     \hline
%     Ours-Bert & 76.80 & 78.65 & 86.40 & 86.95 & 84.88 & 85.77 & 87.50 & 89.79 & 83.90 & 85.29\\
%     Ours-RoBerta & 79.36 & 81.65 & 85.49 & 86.87 & 84.09 & 86.00 & 82.91 & 87.84 & 82.96 & 85.59\\
%     \hline
%     N.P. Bert & \multicolumn{2}{c|}{84.52} & \multicolumn{2}{c|}{90.65} & \multicolumn{2}{c|}{90.61} & \multicolumn{2}{c|}{92.31} & \multicolumn{2}{c}{89.52}\\
%     \hline
%     N.P. RoBerta & \multicolumn{2}{c|}{86.19} & \multicolumn{2}{c|}{91.20} & \multicolumn{2}{c|}{91.64} & \multicolumn{2}{c|}{93.69} & \multicolumn{2}{c}{90.68}\\
%     \hline
%     \hline
%     $\epsilon =$ (MA) & 3 & 8 & 3 & 8 & 3 & 8 & 3 & 8 & 3 & 8\\
%     \hline
%     $\epsilon \approx$ (GDP+CLT) & 2.52 & 5.83 & 2.53 & 5.85 & 2 & 4.75 & 1.73 & 4.33 & <2.53 & <5.85\\
%     \hline
%     \end{tabular}
%     \caption{Compare with others based on DP-SGD}
%     \label{table: DPSGD}
% \end{table*}


% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{cc|cc|cc|cc}
%     \hline
%     \multirow{2}{*}{Models} & \multirow{2}{*}{Layer} & \multicolumn{2}{c|}{SST-2} & \multicolumn{2}{c|}{IMDB} & \multicolumn{2}{c}{AGnews}\\
%     \cline{3-8}
%     & & $\epsilon=1$ & $\epsilon=4$ & $\epsilon=1$ & $\epsilon=4$ & $\epsilon=1$ & $\epsilon=4$\\
%     \hline
%     \multirow{6}{*}{Bert} & 2 & 74.66 & 80.39 & 75.64 & 82.54 & 69.95 & 82.39\\
%     & 4 & 78.56 & 82.11 & 76.62 & 83.83 & 70.21 & 82.03\\
%     & 6 & 79.24 & 83.83 & 76.85 & 84.11 & 70.21 & 82.65\\
%     & 8 & 82.22 & 87.39 & 78.48 & 85.12 & 70.53 & 83.15\\
%     & 10 & 82.45 & 85.67 & 78.05 & 86.30 & 70.72 & 83.62\\
%     & 12 & 82.45 & 88.88 & 79.24 & 87.42 & 70.96 & 83.23\\
%     \hline
%     \multirow{6}{*}{Albert} & 2 & 78.90 & 83.26 & 75.70 & 83.59 & 70.66 & 82.29\\
%     & 4 & 80.96 & 84.98 & 77.17 & 83.43 & 70.53 & 82.29\\
%     & 6 & 81.88 & 86.58 & 78.53 & 84.00 & 70.97 & 82.96\\
%     & 8 & 80.73 & 84.17 & 78.96 & 86.35 & & 83.51\\
%     & 10 & 78.44 & 85.89 & 78.97 & 84.88\\
%     & 12 & 80.39 & 81.19 & 78.89 & 86.15\\
%     \hline
%     \multirow{3}{*}{Distilbert} & 2 & 76.61 & 80.96 & 75.43 & 81.52 & 70.46 & 82.16\\
%     & 4 & 79.24 & 84.17 & 77.20 & 84.71 & 70.20 & 82.37\\
%     & 6 & 81.54 & 87.16 & 78.92 & 86.15 & 70.43 & 82.63\\
%     \hline
%     \end{tabular}
%     \caption{Performance by layer}
%     \label{table: layer}
% \end{table*}

% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{c|cccc}
%     \hline
%     Sensitivity & SST-2 & IMDB & AGnews & QNLI\\
%     \hline
%       1 & 82.34  & 79.63 & 70.46 & 82.26\\
%       0.9 & 81.65 & 79.24 & 70.96 & 82.15\\
%       0.7 & 82.45 & 78.52 & 70.61 & 81.12\\
%       0.5 & 77.87 & 78.67 & 70.47 & 81.12\\
%       0.3 & 81.42 & 79.09 & 70.42 & 81.22\\
%       0.1 & 78.10 & 76.26 & 68.72 & 75.52\\
%     \hline
%     Null Privacy & 92.31 & 89.01 & 93.26 & 90.61\\
%     \hline
%     \end{tabular}
%     \caption{Bert: Fix $\epsilon=1$ and training steps$=\frac{epoch=1}{p}$, accuracy of different sensitivity and noise.}
%     \label{table: GS-noise-acc}
% \end{table*}

% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{c|cccc}
%     \hline
%     Batch & SST-2 & IMDB & AGnews & QQP\\
%     \hline
%       16 & 84.29 & 80.80 & 78.68 & 84.53\\
%       32 & 82.45 & 79.24 & 70.96 & 81.25\\
%       64 & 76.83 & 67.45 & 58.62 & 80.84\\
%     \hline
%     Null Privacy & 92.31 & 89.01 & 93.26 & 90.65\\
%     \hline
%     \end{tabular}
%     \caption{Bert: Fix $\epsilon=1$ and training steps$=\frac{epoch=1}{p}$, accuracy of different batch size.}
%     \label{table: GS-noise-acc}
% \end{table*}



% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{cc|cc}
%     \hline
%     Compose-level & Sensitivity & SST-2 & IMDB \\
%     \hline
%     & 1 & 80.05(0.75) & 74.88(0.87) \\ 
%      & 0.9 & 80.39(0.67) & 78.89(0.78)\\
%      & 0.7 & 74.31(0.52) & 75.00(0.61)\\
%     Dataset & 0.5 & 67.20(0.37)& 76.07(0.44)\\
%      & 0.3 & 66.28(0.22) & 65.00(0.26)\\
%      & 0.1 & 72.59(0.07) & 60.18(0.09)\\
%     \hline
%     \multicolumn{2}{c|}{Null Privacy} & 91.86 & 88.12\\
%     \hline
%     \end{tabular}
%     \caption{Albert: Fix $\epsilon=1$ and training steps$=\frac{epoch=1}{p}$, accuracy of different sensitivity and noise.}
%     \label{table: GS-noise-acc}
% \end{table*}

% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{cc|cc}
%     \hline
%     Compose-level & Sensitivity & SST-2 & IMDB \\
%     \hline
%      & 1 & 79.82(0.75) & 76.90(0.87) \\ 
%      & 0.9 & 81.08(0.67) & 78.92(0.78) \\
%      & 0.7 & 80.16(0.52) & 78.37(0.61)\\
%     Dataset & 0.5 & 80.50(0.37) & 75.81(0.44)\\
%      & 0.3 & 81.54(0.22) & 78.14(0.26)\\
%      & 0.1 & 76.83(0.07) & 75.88(0.09)\\
%     \hline
%     \multicolumn{2}{c|}{Null Privacy} & 90.83 & 91.18\\
%     \hline
%     \end{tabular}
%     \caption{DistillBert: Fix $\epsilon=1$ and training steps$=\frac{epoch=1}{p}$, accuracy of different sensitivity and noise.}
%     \label{table: GS-noise-acc}
% \end{table*}

% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{cc|cccc}
%     \hline
%     Model & $\epsilon$ & IMDB & AGnews & DBpedia & SNLI \\
%     \hline
%     \multirow{3}{*}{Bert} & 1 & 79.63 & 70.96 & 75.68 & 80.01 \\
%     & 2.5 & 82.68 & 80.25 & 86.73 & 83.81 \\
%     & 4 & 87.42 & 83.23 & 87.11 & 85.23 \\
%     \hline
%     \multicolumn{2}{c|}{Null Privacy} & 89.01 & 93.26 & 99.52 & 89.98\\
%     \hline
%     \multirow{3}{*}{RoBerta} & 1 & 76.66 & 70.30 & 75.45 & 80.40 \\
%     & 2.5 & 82.04 & 80.04 & 84.12 & 84.67\\
%     & 4 & 85.22 & 82.76 & 86.88 & 85.49\\
%     \hline
%     \multicolumn{2}{c|}{Null Privacy} & 90.32 & 93.81 & 99.60 & 90.78\\
%     \hline
%     \end{tabular}
%     \caption{Different tasks}
%     \label{table: Different tasks}
% \end{table*}

% \begin{table*}[htp!]
%     \centering
%     \begin{tabular}{c|c|ccc|ccc}
%     \hline
%     \multirow{3}{*}{Models} & \multirow{3}{*}{$\epsilon$} & \multicolumn{3}{c|}{Accuracy on \textbf{SST-2}} & \multicolumn{3}{c}{Accuracy on \textbf{IMDB}} \\
%     \cline{3-8}
%     & & All-data & All-data & One-step & All-data & All-data & One-step\\
%     & & \small{w/o amplification} & \small{w/ amplification} & \textbf{Wrong} & \small{w/o amplification} & \small{w/ amplification} & \textbf{Wrong}\\
%     \hline
%     \multirow{2}{*}{Bert} & 1 & 59.40(2.53) & 82.45 (0.52) & 90.37 (0.266) & 58.79(3.07) & 79.24(0.78) & 89.38(0.315)\\
%     & 4 & 74.77(0.74) & 88.88(0.34) & 90.14(0.205) & 76.22(0.91) & 87.42(0.48) & 88.04(0.276)\\
%     C=0.7|0.9 & 8 & 86.12(0.41) & 90.60(0.3) & 90.83(0.195) & 88.42(0.42) & 86.77(0.51) & 88.90(0.262)\\
%     \hline
%     \multirow{2}{*}{Albert} & 1 & 57.57(3.26) & 80.39(0.67) & 86.58(0.296) & 57.94(3.07) & 78.89(0.78) & 88.83(0.315)\\
%     & 4 & 72.82(0.94) & 81.19(0.44)& 84.86(0.263) & 70.35(0.91) & 86.15(0.48) & 88.66(0.276)\\
%     C=0.9 & 8 & 82.91(0.53) & 86.24(0.39)& 83.60(0.25) & 84.95(0.51) & 87.19(0.41) & 88.40(0.262)\\
%     \hline
%     \multirow{2}{*}{Distilbert} & 1 & 59.40 & 81.54 & 88.19 & 58.15 & 78.92 & 89.02\\
%     & 4 & 75.57 & 87.16 & 88.76 & 76.18 & 86.15 & 88.46\\
%     C=0.9 & 8 & 84.75 & 89.68 & 90.02 & 84.94 & 88.10 & 88.95\\
%     \hline
%     \end{tabular}
%     \caption{(Copy) Performance by composition}
% \end{table*}

